Cost-Effective Data Feeds to Blockchains via Workload-Adaptive Data Replication

Feeding external data to a blockchain, a.k.a. data feed, is an essential task to enable blockchain interoperability and support emerging cross-domain applications, notably stablecoins. Given the data-intensive feeds in real life (e.g., high-frequency price updates) and the high cost in using blockchain, namely Gas, it is imperative to reduce the Gas cost of data feeds. Motivated by the constant-changing workloads in finance and other applications, this work focuses on designing a dynamic, workload-aware approach for cost effectiveness in Gas. This design space is understudied in the existing blockchain research which has so far focused on static data placement. This work presents GRuB, a cost-effective data feed that dynamically replicates data between the blockchain and an off-chain cloud storage. GRuB's data replication is workload-adaptive by monitoring the current workload and making online decisions w.r.t. data replication. A series of online algorithms are proposed that achieve the bounded worst-case cost in blockchain's Gas. GRuB runs the decision-making components on the untrusted cloud off-chain for lower Gas costs, and employs a security protocol to authenticate the data transferred between the blockchain and cloud. The overall GRuB system can autonomously achieve low Gas costs with changing workloads. We built a GRuB prototype functional with Ethereum and Google LevelDB, and supported real applications in stablecoins. Under real workloads collected from the Ethereum contract-call history and mixed workloads of YCSB, we systematically evaluate GRuB's cost which shows a saving of Gas by 10% ~ 74%, with comparison to the baselines of static data-placement.

==> sty/llncs2e/titlepage.tex <==
\input{sty/title.tex}
\author{
Kai Li\hspace{0.25cm}
Yuzhe (Richard) Tang\hspace{0.25cm}
Beom Heyn (Ben) Kim$\ ^\dag{}$\hspace{0.25cm}
Jianliang Xu$\ ^\ddag{}$\hspace{0.25cm}\\
\ifdefined\TTUT
\fi
}

\institute{
    \fontsize{10}{10}\selectfont\itshape
    Syracuse University, New York, USA\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag{}$University of Toroto, Ontario, Canada\\
    \fontsize{10}{10}\selectfont\itshape
    $^\ddag{}$Hong Kong Baptist University, Kowloon Tong, Hong Kong 
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/titlepage.tex <==
\input{sty/title.tex}
\author{
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/usepackage.tex <==
\usepackage{etoolbox}
\makeatletter
\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
\makeatother

\usepackage{titlesec}
{\filcenter\normalfont\Large\bfseries}
\titleformat{\chapter}
  {\normalfont\sffamily\LARGE\it}
  {\thechapter.}{10pt}{\LARGE}
\titlespacing*{\chapter}{0pt}{0pt}{0pt}
\titleformat{\section}
  {\normalfont\sffamily\Large\bfseries}
  {\thesection.}{0.3em}{}
\titleformat{\subsection}
  {\normalfont\sffamily\large\it}
  {\thesubsection.}{0.3em}{}





==> sty/sig-alternate/titlepage.tex <==
\input{sty/title.tex}
%\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

%\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\ifdefined\TTUT
\numberofauthors{4} % if number of authors is bigger than number of \alighauthor used following, a ``addtional author'' section will be shown in the end of the paper.
%note: no empty line!
\author{
\alignauthor
Yuzhe Tang$^\dag$
%\titlenote{Author notes}
\\       \affaddr{Syracuse University}
\\       \affaddr{Syracuse, NY 13244}
\\       \email{$^\dag$ytang100@syr.edu}
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\and
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
}
\date{30 July 1999}
\fi
\maketitle



==> sty/sig-alternate/titlepage_sharedAuthorAddr.tex <==
\begin{document}
%
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
%
\linespread{0.9}

% --- Author Metadata here ---
\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\title{
Tang's Template of IEEEtran.cls for Conferences \titlenote{!Eye-catching title for high citation: make it short}
}

\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\numberofauthors{1}
\author{
\alignauthor Yuzhe Tang, Ting Wang and Ling Liu \\
  \affaddr{College of Computing, Georgia Institute of Technology} \\ 
  \affaddr{ Atlanta, GA 30332, USA} \\
  \email{yztang@gatech.edu, \{twang, lingliu\}@cc.gatech.edu}
}
\date{30 July 1999}
\maketitle



==> sty/title.tex <==
\begin{document}
% --- Author Metadata here ---
\title{
Cost-Effective Data Feeds to Blockchains via Workload-Adaptive Data Replication
\\ {\large \today}
\ifdefined\TTTOME
Tang's Paper Template \\ Title to be eye-catching for high citation: \\what's new \\short, \\mention approach (to researcher audience)
\fi
}


==> sty/usenix/titlepage.tex <==
\input{sty/title.tex}

\ifdefined\TTUT
\author{
{\rm Your N.\ Here}\\
Your Institution
\and
{\rm Second Name}\\
Second Institution
% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
} % end author
\fi

\maketitle

% Use the following at camera-ready time to suppress page numbers.
% Comment it out when you first submit the paper for review.
\thispagestyle{empty}





==> sty/usenix/usepackage.tex <==
\usepackage{sty/usenix/usenix,epsfig,endnotes}


==> text/discuss.tex <==
\section{Discussion}

\subsection{Case Study: Verifying Cloud-Storage Consistency}

A smart contract can audit cloud logs to verify the cloud operation consistency and to enforce service-level agreement (SLA)~\cite{DBLP:conf/fc/Bonneau16a,DBLP:journals/corr/abs-1904-06626}. In this application, the monitored system is a cloud service with multiple concurrent clients, where they initially agree on an SLA. The log-auditing smart contract is fed with a stream of concurrent operations collected from different clients. The contract maintains a state of the latest snapshot of cloud storage. Upon the arrival of a new operation, the contract runs consistency algorithms~\cite{DBLP:conf/sosp/LuVAHSTKL15} that solve the total-order among operations and find inconsistency anomaly. If there is no inconsistency found, the contract would append the current operations to the state.

There are other domain scenarios that the smart contract needs to run stateful computation. For instance, data analytics on public datasets commonly require public auditability and carrying them out in smart contract to increase data transparency and computation integrity. This contract-based analytics paradigm can be applied to data sharing in public sectors for applications in smart cities, medical data research, etc.

\ifdefined\TTUT
\subsection{Infeasibility to Token Contracts}

An important application of smart contract is token systems (e.g., ERC20 standards). Briefly, a token contract is called by a token owner to transfer her tokens to another owner. To do so, the token contract often maintains as a state the balance sheet of all owners (or their addresses). In the state, each entry is the list of tokens that an address currently owns. A transfer call, say from address A to B, results in a state update that A's balance is deducted and B's balance is increased. In other words, a transfer call needs to read-modify-write the state of token contract. And the read-write ratio is always 1:1.

When placing the state on-chain, the most expensive operation is contract-storage write (in the read-modify-write sequence), whose unit cost is $5000$ per word. When placing the state off-chain, the most expensive operation is transfer fee caused by the read (as in the read-modify-write sequence), whose unit cost is $2167$ per word. Thus, under $1:1$ read-write ratio, the cost difference between the two strategies (on-chain or off-chain storage) is not significant.\footnote{We also considered batching operations in a transaction, which does not result in large cost difference.} Our experiment results in Figure~\cite{XXX} also corroborates the observation. This analysis shows that token contracts may not be a good application for GRuB. 
\fi



==> text/lst21.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}

//TokenContract_ImmediateValidate

bool DO_transfer(address[] buyers, address[] sellers, uint256[] tokens){
     // validate transfer() before sending it to Blockchain.
     Puts(transfer, buyers, sellers, tokens);
}

KV Callback(int funcName, KV records){
     Assert(funcName == getBalance);
     If(grubStorageContract.balance[buyer] >= 0)
         return records;
     ViolationPolicy.reportNegativeBalance();
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Application contract supporting ERC20 tokens with deferred validation}
\label{lst:appcontract:token:deferred}
\end{figure}


==> text/lst22.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
// Off-chain client extension
void DOTransfer(address from, address to, uint tokens){
    balanceFrom = GetQ(from);
    balanceTo = GetQ(to);
    if(balanceFrom >= tokens){
        localKV.push(from,balanceFrom-token);
        localKV.push(from,balanceTo+token);
    }
    if (time - lastEpoch > epochSize){
        GRuB.Puts(localKV);
        localKV.clear();
    }
}

unit DUBalanceOf(address owner){
    balance = GetQ(owner);
    return balance;
}

// On-chain application contract
uint EvalQ(unit balance){
    return balance;
}

\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Application contract supporting ERC20 tokens}
\label{lst:appcontract:token}
\end{figure}


==> text/lst3.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
// On off-chain DO 
void issueCert(Cert cert){
    if(vrfy(cert, pubKeyCA)){
        localKV.push(cert.hostname, cert);
        if(time - lastEpoch > epochSize){
            GRuB.Puts(localKV);
            localKV.clear(); }}}

// On off-chain DU
void auditCert(String hostname, Cert[] localCerts){
    GRuB.GetQ(hostname, SHA256(localCerts), AuditLogOnchain); }

// In application contract on-chain
bool auditLogOnchain(Cert[] matchCerts, HashDigest d){
    return SHA256(matchCerts) == d;}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Application contract supporting CT log auditing}
\label{lst:ctlogcontract}
\end{figure}


==> text/more_eval.tex <==
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures_kai_macro/exp-Gasperoperation-YCSB-memoryless-eps-converted-to.pdf}
\end{center}
%\vspace{-0.15in}
\caption{GRuB under YCSB workload with changing read-write patterns}
\label{fig:macro:1}
\vspace{-0.10in}
\end{figure}



In this experiment, we evaluate the gas cost of GRuB under YCSB workloads. In particular, we modified the read/write portion in workload E to generate three sequences of operations, containing 5\%, 80\%, 5\% reads respectively. We use the memoryless algorithm in GRuB and compare its gas cost with the strategy of always replicating data (Baseline BL1), and the strategy of never replicating data (Baseline BL2). Here the reported metric is the average gas cost of operations in a read-write sequence. Here, a read-write sequence is defined to be such that it starts with consecutive writes followed by consecutive read operations. The result, presented in Figure~\ref{fig:macro:1}, shows that in the first phase, namely from sequence 1 to sequence 65, when the sub-workload contains 5\% reads, the gas cost of GRuB is similar to the cost of BL2. The costs of both schemes are $1/5$ of that of BL1. In this write-intensive phase, BL2 is optimal, and our GRuB online algorithm consistently produces the $NR$ decisions, similar to the optimal BL2. In the second phase where the trace contains 80\% reads (from sequence 66 to sequence 135), the online algorithm in GRuB makes decisions $R$, and achieves the Gas cost $1/8$ of that of BL2. Compared with BL1, which is the optimal scheme in this phase, GRuB's cost decreases and then stops at two times of the cost of BL2. In the third phase, the sub-workload has a similar read portion with the first phase. The gas costs of the three schemes are similar in the beginning and after convergence, GRuB achieves similar gas costs with BL2, and the gas costs of both schemes are $1/5$ of that of BL1. 
The experiment shows the effectiveness of GRuB adapting to a changing workload.



    \subfloat[Varying parameter $K$ (YCSB)]{%
        \includegraphics[width=0.15\textwidth]{figures_kai_macro/exp-Gasperoperation-ParameterK-eps-converted-to.pdf}
        \label{fig:macro:2}%
    }




==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table*}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

\subsection{figures}
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5-eps-converted-to.pdf}
\caption{Wrapped figure}
\label{fig:perf}
\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5-eps-converted-to.pdf}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5-eps-converted-to.pdf}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2-eps-converted-to.pdf}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10-eps-converted-to.pdf}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
		...
		*Bitmap bm = BitmapFactory.decodeFile(file)*;
		return bm;
}

void EditPicture(Bitmap bm) {
		//heavy computational picture editing
		bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
		for(every pixel) {
			...
		}	
		
		//embed location information into picture
		*Location loc = getLastKnownLocation(Provider)*;
		*double longitude = loc.getLongitude()*;
		*double latitude = loc.getLatitude()*;
		*EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}
\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}
\end{center}



\subsection{misc}
\begin{itemize}
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

